TURJUMAN: A Public Toolkit for Neural Arabic Machine Translation

We present TURJUMAN, a neural toolkit for translating from 20 languages into Modern Standard Arabic (MSA). TURJUMAN exploits the recently-introduced text-to-text Transformer AraT5 model, endowing it with a powerful ability to decode into Arabic. The toolkit offers the possibility of employing a number of diverse decoding methods, making it suited for acquiring paraphrases for the MSA translations as an added value. To train TURJUMAN, we sample from publicly available parallel data employing a simple semantic similarity method to ensure data quality. This allows us to prepare and release AraOPUS-20, a new machine translation benchmark. We publicly release our translation toolkit (TURJUMAN) as well as our benchmark dataset (AraOPUS-20).

==> S2S_LM.tex <==
\section{Pretrained Language  Models}\label{sec:LM} 
In this section we will present the Arabic and multilingual generative  models which  can be utilized to solve summarization,  question answering, and machine translation.



\noindent\textbf{mBART50}~\cite{liu2020multilingual} is a multilingual generative (sequence-to-sequence)  model primarily intended for translation task. mBART trained by denoising full texts in 50 languages (including Arabic). Then, mBART is fin-tuned on parallel MT data under three settings:: Many-to-English, English-to-Many and Many-to-Many. The parallel MT data used contains a total of 230M parallel sentences and covers high-, mid-, and low resourced languages.

\noindent\textbf{mT5}~\cite{xue2020mt5} is the multilingual version of \textbf{T}ext-\textbf{t}o-\textbf{T}ext \textbf{T}ransfer \textbf{T}ransformer model (T5)   \cite{raffel2019exploring}.   The basic idea behind  this  model is to  treat every  text-based language task as a “text-to-text” problem, (i.e. taking text format as input and producing new text format as output), where   a multi-task learning  is applied to several  NLP tasks: question answering, document summarization, and machine translation.  mT5  is trained on the ``mC4: Multilingual Colossal Clean Crawled Corpus", which is  $\sim26.76$TB for $101$ languages (including Arabic). 

\noindent\textbf{AraT5}~\cite{nagoudi2022_arat5} is an  Arabic text-to-text Transformer  model dedicated to MSA and its dialects. It is essentially an encoder-decoder Transformer similar in configuration and size to T5 \cite{raffel2019exploring}.  AraT5 is trained on more than $248$GB of Arabic text ($70$GB MSA and $178$GB tweets). 
